Negation-Instance Based Evaluation of End-to-End Negation Resolution

In this paper, we revisit the task of negation resolution, which includes the subtasks of cue detection (e.g. "not", "never") and scope resolution. In the context of previous shared tasks, a variety of evaluation metrics have been proposed. Subsequent works usually use different subsets of these, including variations and custom implementations, rendering meaningful comparisons between systems difficult. Examining the problem both from a linguistic perspective and from a downstream viewpoint, we here argue for a negation-instance based approach to evaluating negation resolution. Our proposed metrics correspond to expectations over per-instance scores and hence are intuitively interpretable. To render research comparable and to foster future work, we provide results for a set of current state-of-the-art systems for negation resolution on three English corpora, and make our implementation of the evaluation scripts publicly available.

==> backlog.tex <==
\textbf{Downstream task perspective:}\annetodo{Need to integrate these points somewhere earlier in the paper}
\begin{itemize}
\item FUTURE WORK: open IE: which relations should be negated? - negation automatically integrated? - RQ: how can negation (like conditions) shown in a more principled way in IE?
\end{itemize}

		\begin{tabular}{l}
		
		\blue{\textbf{(1) No Scope:}}\\ %
		\textbf{Gold:}\hspace{6.2mm} If \textbf{not} , I 'll have to do with you .\\
		\textbf{Predicted:} If \textbf{not} \underline{\smash{\red{, I 'll have}}} to do with you .\\
		$\rightarrow$ \textit{Token-wise minor impact on overall precision score}\\
		\textit{but severe impact on potential applications.}\\
	    \vspace{2mm}\\
	    
	    [He made \textbf{no} remark], but the matter remained in his thoughts.\\
	
	    \blue{\textbf{(2) Long Scope} (with relative clause and complement):}\\
	    \textbf{Gold}: `` Well , Mrs. Warren , I can see that you have any\\
	    particular cause for , \textbf{nor} \underline{\smash{do}}\underline{\smash{ I}}\underline{\smash{ understand}}\underline{\smash{ why}}\underline{\smash{ I}}\underline{\smash{ ,}}\underline{\smash{ whose}}\\
	    \underline{\smash{ time}}\underline{\smash{ is}}\underline{\smash{ of}}\underline{\smash{ some}}\underline{\smash{ value}}\underline{\smash{ ,}}\underline{\smash{ should}}\underline{\smash{ interfere}}\underline{\smash{ in}}\underline{\smash{ the}}\underline{\smash{ matter}} .\\
	    
	    \textbf{Pred.}: `` Well , Mrs. Warren , I can see that you have any\\
	    particular cause for , \textbf{nor} \underline{\smash{do}}\underline{\smash{ I}}\underline{\smash{ understand}}\underline{\smash{ why}}\underline{\smash{ I}}\underline{\smash{ ,}} \red{whose}\\
	    \red{time is of some value ,} \underline{\smash{should}}\underline{\smash{ interfere}} \red{in the matter} .\\
		$\rightarrow$ \textit{Token-wise notable impact on overall recall score,}\\
		\textit{but should we punish a system for such a response?}
		\end{tabular}
		

\textbf{Brainstorming Stefan/Anne}
\begin{itemize}
\item Idee: nur ConanDoyle (Name aus Original papier)
\item Tasks + Metriken (linguistische Motivation darstellen)
\item Diskussion: what is really evaluated / important? Blanco und Moldovan: logik level vs. semantisch/pragmatisch
\item Ergebnisse für Top System auf CD En und CN
\end{itemize}


\paragraph{Research Questions and Hypotheses.}
\begin{enumerate}
    \item We test different dependency-based representations for negation/speculation resolution. (Comparison with NegBERT / sequence tagging approaches)
    \item Analyse forest of evaluation metrics and unify evaluation of recently proposed transformer-based approaches to negation resolution.
    \item Take a step back and re-consider what really matters for evaluating negation: illustrate weaknesses of existing metrics, do we have a linguistically motivated suggestion how to improve?
    \item Does multi-task learning with UD help? \red{(very tiny side question)}
    \item Analyse (especially for the graph type integrating syntax) which cases work well, go wrong, etc. (for which types of syntactic constructions is negation/speculation resolution easy/difficult for the system?) $\rightarrow$ automatically create a test suite for different types of constructions \cite{ribeiro-etal-2020-beyond} - I think something like this (breaking down performance by syntactic construction) has been done in the context of NLI
    \item what is the effectiveness of neural language models? to what extent do they capture negation - e.g., look at representation of affirmative vs. negated version, are there explainability / BERTology papers that looked at this? if yes cite, if no, can we look at it?
\end{enumerate}


Meeting May 19
\begin{itemize}
    \item analysing evaluation metrics w.r.t. to linguistic vs. application perspective
    \item different data sets use different schemes, cross-domain experiments have limited expressiveness (?)
    \item providing a clean version of the SOTA models' results (including our own new model)
    \item provide additional diagnostic tests, minimal pairs (constructed examples), CHECKLIST, ... -- start with automatically generated cases or sentences from linguistics textbook, completely controlled evaluation set, ambiguous vs. unambiguous cases
    \begin{itemize}
        \item negation of clauses vs. constituents (nominal vs. verbal, ...)
        \item affixes vs. single vs. multi-cues
        \item length of scope
        \item alignment with constituent structure
        \item effects of focus?
        \item nested scopes
        \item punctuation (see Fancellu)
        \item continous vs. discontinuous scopes
    \end{itemize}
\end{itemize}


\textbf{Concrete example:} Liza's multi-word cue example, where Anne thinks that there are 3 negated events kind of in parallel.
Annotation is as a multi-word-cue with a single scope and event.
The system predicted three scopes.
\blue{The name "scope" is also odd, actually, for me, scope is always a scope of something, here the negation cue.}



Would an event-semantic interpretation help here?
Compare to meaning-banking approaches: do they have the same issues? Has negation resolution been addressed specifically on meaning banks such as the Groningen meaning bank? The \citet{jimenez-zafra-etal-2020-corpora} survey mentions these treebanks as corpora annotated for negation ...
If yes how was negation resolution evaluated?

What about treatment in semantic parsing approaches?

\citet{blanco2011some}: very instructive summary of negation in natural language and how to create semantic representations (from a high level point of view)
If we don't have focus annotations, we possibly cannot construct the correct semantic representations, we only know that the sum (composition) of all the elements in the scope evaluates to false.

\textbf{Discussion Anne, Liza:}
Problematic: Multi-word cues (neither...nor) are annotated as a single cue with a single scope, but in the case we can imagine, they should actually have two differing scopes.
\red{Re-annotate ConanDoyle discontinuous multiword cue (neither nor) sentences? - overlapping discontinuous scopes - goal: more meaningful annotation} TODO: check literature on negated coordinations
What to do if the model predicts them as separate cues, given the simplifying annotations in the data?


\textbf{Ideas for metrics that make sense:}\\
\textbf{Evaluation of scope detection:}\\
categorize into standard main scores + variants\\
all our metrics are motivated by \underline{negation instance} - level evaluation\\
\begin{itemize}
    \item \textbf{Cue detection}: F1 on cue level (per negation instance!) (strict vs. partial match vs. head match): discussion: task truth-theoretic perspective: recognize there is sth. going on in the sentence; for linguistics / pragmatics / real machine comprehension, the "longer" matters as well -- extra-propositional implications (current downstream tasks rarely capture these)
    \item \textbf{scope resolution, Gold cues given}:
    \begin{itemize}
        \item PCS percentage of correct scopes (matched fully / exactly as in the gold corpus) \lizatodo{should correspond to recall of scope-level scope} %
        \item scope resolution, Gold cues given: F1 for token-level scope matching (however, STs do this by sentence, shouldn't we do this by negation instance (scope) and then average?) - even if nested scopes: they would count as two scopes \blue{mathematical difference vs. existing metrics?}
    \end{itemize}
    \item \textbf{end-to-end}: also based on negation instances
    \begin{itemize}
        \item "Negated": Full Negation (everything needs to be correct per negation instance): with/without Events (reasoning: how events are expressed in text is a different question); \lizatodo{different from *SEM 2012 "negated" where it refers to events specifically} %
        \item End to end score: only relevant for downstream perspective: \textit{What if there is an overlap of scopes, but cue not correctly linked?} Evaluation as in dependency parsing? \red{TODO: discuss next week?}
    \end{itemize}
    \item Proposal for new score: precision and recall on edges. Argumentation: both for logical and downstream perspective, scope without marker is not really useful: Katja did \textit{not} enter the house (today). Katja did \textit{never} enter the house (ever). not(enter(Katja, house)), forall s not(Katja(enter, house)), I am not angry. vs. I am never angry. - "units of meaning"? event or sth that has a referent
    \item Dependency parsing based approach: from annotated corpus to eval. structure (negation backbone?): find head verb of negated element, find arguments + complements: create edges from Neg. cue to these nodes. syntax as a proxy for semantic roles. F1 on edges, (compute per sent., then average ?) -- not one score, but plot over sentence length / number of edges, edges count as correct either if head has been detected correctly, or if entire span belonging to the "node" is correct; (surface oriented vs. semantics oriented)
    \item we only have automatic parses: map to annotation of negation scopes, if it doesn't fit: correct manually
    \item Focus: propose sth. that counts only as correct if everything including focus has been marked correctly? \red{if there was a dataset that annotated both ... i.e., in the future :)} linguistics might actually care about this complete version even more ...
\end{itemize}




\begin{table}[h]
    \centering
    \footnotesize
    \begin{tabular}{lrrrrr}
        \toprule
         & \textbf{CT} & \textbf{CS} & \textbf{ST} & \textbf{FN} \\
        \toprule
        \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textit{Negation}} \\
        \midrule
        \citet{britto2020resolving} & 87.32 & - & 91.25 & - \\
        \citet{khandelwal-britto-2020-multitask} & 87.07 & - & 93.19 & - \\
        Ours & & & & \\
        \midrule
        \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textit{Speculation}} \\
        \midrule
        \citet{britto2020resolving} & 92.66 & - & 91.00 & - \\
        \citet{khandelwal-britto-2020-multitask} & 92.61 & - & 91.35 & - \\
        Ours & & & & \\
        \bottomrule
    \end{tabular}
    \caption{SFU results. CT = Cue (Token-level), CS = Cue (Scope-level), ST = Scope (Token-level), FN = Full Negation}
    \label{tab:sfu_results}
\end{table}
